ORCNet: A context-based network to simultaneously segment the ocular region components

Accurate extraction of the Region of Interest is critical for successful ocular region-based biometrics. In this direction, we propose a new context-based segmentation approach, entitled Ocular Region Context Network (ORCNet), introducing a specific loss function, i.e., he Punish Context Loss (PC-Loss). The PC-Loss punishes the segmentation losses of a network by using a percentage difference value between the ground truth and the segmented masks. We obtain the percentage difference by taking into account Biederman's semantic relationship concepts, in which we use three contexts (semantic, spatial, and scale) to evaluate the relationships of the objects in an image. Our proposal achieved promising results in the evaluated scenarios: iris, sclera, and ALL (iris + sclera) segmentations, utperforming the literature baseline techniques. The ORCNet with ResNet-152 outperforms the best baseline (EncNet with ResNet-152) on average by 2.27%, 28.26% and 6.43% in terms of F-Score, Error Rate and Intersection Over Union, respectively. We also provide (for research purposes) 3,191 manually labeled masks for the MICHE-I database, as another contribution of our work.

==> text/acknowledgments/text.tex <==
%!TEX root = ../../main.tex


% use section* for acknowledgment
\ifCLASSOPTIONcompsoc
  % The Biometrics Council usually uses the plural form
  \section*{Acknowledgments}
\else
  % regular IEEE prefers the singular form
  \section*{Acknowledgment}
\fi


This work was supported by grants from the National Council for Scientific and Technological Development~(CNPq) (\#~428333/2016-8, \#~313423/2017-2 and \#~307277/2014-3) and the Coordination for the Improvement of Higher Education Personnel~(CAPES). 
The Titan V GPUs used for this research were donated by the NVIDIA Corporation. 

==> text/appendices/text.tex <==
%!TEX root = ../../main.tex


\appendices
\section{Proof of the First Zonklar Equation}
Appendix one text goes here.

% you can choose not to have a title for an appendix
% if you want by leaving the argument blank
\section{}
Appendix two text goes here.

==> text/authors/text.tex <==
%!TEX root = ../../main.tex


% biography section
% 
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:

% insert where needed to balance the two columns on the last page with
% biographies
%=\newpage

% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}




\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/authors/diego.jpeg}}]{Diego Rafael Lucio}
is PhD student in Computer Science at UFPR, he is part of the research group VRI (Robotic Vision and Image) of UFPR, working on research on Computer Vision. He holds a degree in Technology and Systems for the Internet by the Universidade Tecnológica Federal do Paraná (2011) and a Master's Degree in Computer Science from the State University of Maringá (2016). He has experience in the area of Computer Science, with emphasis on Computer Vision, working mainly on the following topics: pattern recognition, classification and classification of images.
\end{IEEEbiography}

\vspace{24pt}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/authors/luiz.jpg}}]{Luiz A. Zanlorensi}
is a PhD candidate at the Federal University of Paraná (UFPR), Brazil.
He received his bachelor’s degree in informatic (2013) and a master’s degree in applied computing (2015) from the State University of Ponta Grossa (UEPG),
Brazil.
His research interests include Biometrics, Computer Vision, Machine Learning and Pattern Recognition.
\end{IEEEbiography}

\vspace{24pt}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/authors/yandre.jpg}}]{Yandre M. G. Costa}
 received the B.S. degree in Computer Science from the State University of Maringá(UEM), Maringá, PR, Brazil, in 1997; the M.Sc. degree in Computer Science from the Federal University of Rio Grande do Sul (UFRGS), Porto Alegre, RS, Brazil, in 2002; and Ph.D. degree in Computer Science from the Federal University of Paraná(UFPR), Curitiba, PR, Brazil, in 2013. In 2006 he joined the UEM, where he is a professor of the Department of Informatics and, since 2014, member of the Graduate Program in Computer Science. His current interests include Pattern Recognition, Machine Learning, Image Analysis and Multimedia Retrieval.
\end{IEEEbiography}

\vspace{24pt}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/authors/david.jpeg}}]{David Menotti} is an associate professor at the Department of Informatics, Federal University of Paran\'a, since 2015.
He received his Computer Engineering degree and Master in Applied Informatics from Pontifícia Universidade Católica do Paraná (Brazil) in 2000 and 2003, respectively, and his PhD (in co-tutelle) in Informatics and Computer Science from Université Paris-Est (France) and Universidade Federal de Minas Gerais (Brazil)), respectively,  in 2008. 
He was with the Computing Department, Universidade Federal de Ouro Preto (Brazil) from 2008 to 2015. 
He spent his sabbatical year (2013-2014) at the Institute of Computing, University of Campinas as a post-doctoral researcher. 
His research interests are Computer Vision, Pattern Recognition, Machine Learning and Image Processing.
\end{IEEEbiography}

\balance
